AlphaRouter: Quantum Circuit Routing with Reinforcement Learning and Tree Search

Quantum computers have the potential to outperform classical computers in important tasks such as optimization and number factoring. They are characterized by limited connectivity, which necessitates the routing of their computational bits, known as qubits, to specific locations during program execution to carry out quantum operations. Traditionally, the NP-hard optimization problem of minimizing the routing overhead has been addressed through sub-optimal rule-based routing techniques with inherent human biases embedded within the cost function design. This paper introduces a solution that integrates Monte Carlo Tree Search (MCTS) with Reinforcement Learning (RL). Our RL-based router, called AlphaRouter, outperforms the current state-of-the-art routing methods and generates quantum programs with up to $20\%$ less routing overhead, thus significantly enhancing the overall efficiency and feasibility of quantum computing.

==> text/impact.tex <==
\section*{Impact Statement}
This paper contributes to the advancement of quantum computing by introducing an RL-based method for quantum circuit routing. We acknowledge the broader societal implications of quantum technology, including potential impacts on data security and complex problem-solving. There are many potential societal consequences of improving quantum computing.

==> text/recycle.tex <==
\begin{figure}[t]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{figures/circuit.pdf}}
\caption{A quantum circuit with five qubits, single-qubit gates and two-qubit gates. Quantum circuits compute by evolving the qubit states via quantum gates. Time goes left to right.}
\label{fig:circuit}
\end{center}
\vskip -0.2in
\end{figure}

\begin{algorithm}[tb]
   \caption{MCTS Placeholder}
   \label{alg:example}
\begin{algorithmic}
   \STATE {\bfseries Input:} data $x_i$, size $m$
   \REPEAT
   \STATE Initialize $noChange = true$.
   \FOR{$i=1$ {\bfseries to} $m-1$}
   \IF{$x_i > x_{i+1}$}
   \STATE Swap $x_i$ and $x_{i+1}$
   \STATE $noChange = false$
   \ENDIF
   \ENDFOR
   \UNTIL{$noChange$ is $true$}
\end{algorithmic}
\label{alg:MCTS}
\end{algorithm}

Algorithm~\ref{alg:MCTS} shows the RL algorithm used for the compiler.
